Pruning Neural Networks at Initialization: Why are We Missing the Mark?

Recent work has explored the possibility of pruning neural networks at initialization. We assess proposals for doing so: SNIP (Lee et al., 2019), GraSP (Wang et al., 2020), SynFlow (Tanaka et al., 2020), and magnitude pruning. Although these methods surpass the trivial baseline of random pruning, they remain below the accuracy of magnitude pruning after training, and we endeavor to understand why. We show that, unlike pruning after training, randomly shuffling the weights these methods prune within each layer or sampling new initial values preserves or improves accuracy. As such, the per-weight pruning decisions made by these methods can be replaced by a per-layer choice of the fraction of weights to prune. This property suggests broader challenges with the underlying pruning heuristics, the desire to prune at initialization, or both.

==> appendices/ablations-at-init.tex <==
\section{Ablations for OMP, SNIP, and GraSP at Initialization}
\label{app:ablations}

In this Appendix, we conduct several ablation studies on one-shot magnitude pruning (OMP), SNIP, and GraSP when applied at initialization to the neural networks from the GraSP paper (Appendix \ref{app:grasp}, Table \ref{tab:grasp-networks}) at the sparsities in the GraSP paper.
Our goal is to understand the specificity of the scores issued by these heuristics and the extent to which the heuristics behave in accordance with the justifications provided by \citet{lee2019snip} and \citet{wang2020picking}.

For each technique, we perform the following experiments with the scores $s$ assigned to the weights by the technique.
\begin{itemize}
    \item The standard version of the technique (marked with a * in each table).
    \item Randomly shuffling the scores within each layer before pruning. This experiment assesses whether the technique is learning which specific parameters to prune or the layerwise proportions by which to prune the network.
    \item Randomly reinitializing the network. This experiment assesses whether the technique is specific to the initial values of the parameters.
    \item Pruning the parameters that the technique considers least important (e.g., pruning parameters with the highest scores if the technique typically prunes the parameters with the lowest scores). This experiment assesses the validity of the mapping between scores and importance.
\end{itemize}

\subsection{One-Shot Magnitude Pruning}

Table \ref{tab:ablation-omp} below conducts the ablations for one-shot magnitude pruning at initialization.
It is possible to randomly shuffle the pruning masks found at initialization and to randomly reinitialize the pruned network without substantial change in accuracy.
This means that, at initialization, OMP is identifying only layerwise proportions in which to prune the network.
It is not identifying the specific sparse structure within each pruned layer or the specific initial weights to retain.
OMP correctly determines that high-magnitude parameters are more important to final accuracy than low-high-magnitude parameters, but it is possible that pruning high-magnitude weights simply selects poor layerwise proportions in which to prune the network.


\begin{table}[h]
%\resizebox{\textwidth}{!}{%
\centering
\small
\begin{tabular}{l | c c c c c}
    \toprule
    Name & Sparsity & Lowest $s$* & Lowest $s$ (Shuffled) & Lowest $s$ (Reinit) & Highest $s$ \\ \midrule
    \multirow{3}{*}{VGG-19}
	 & $90\%$ & $92.8\%$ & $92.8\%$ $(+0.0)$ & $93.0\%$ $(+0.2)$ & $88.4\%$ $(-4.4)$ \\
	 & $95\%$ & $92.4\%$ & $92.4\%$ $(+0.0)$ & $92.4\%$ $(+0.0)$ & $85.3\%$ $(-7.1)$ \\
	 & $98\%$ & $91.6\%$ & $91.6\%$ $(+0.0)$ & $91.7\%$ $(+0.1)$ & $10.0\%$ $(-81.6)$ \\
	 \midrule
    \multirow{3}{*}{WRN-32-2}
	 & $90\%$ & $92.4\%$ & $92.5\%$ $(+0.1)$ & $92.6\%$ $(+0.2)$ & $90.7\%$ $(-1.7)$ \\
	 & $95\%$ & $91.0\%$ & $91.3\%$ $(+0.3)$ & $91.3\%$ $(+0.3)$ & $83.2\%$ $(-7.8)$ \\
	 & $98\%$ & $88.0\%$ & $88.4\%$ $(+0.4)$ & $88.3\%$ $(+0.3)$ & $50.9\%$ $(-37.1)$ \\
	 \midrule
    \multirow{3}{*}{ResNet-50}
	 & $60\%$ & $74.1\%$ & $74.2\%$ $(+0.1)$ & $74.1\%$ $(+0.0)$ & $72.0\%$ $(-2.1)$ \\
	 & $80\%$ & $71.0\%$ & $71.3\%$ $(+0.3)$ & $47.5\%$ $(-23.5)$ & $67.8\%$ $(-3.2)$ \\
	 & $90\%$ & $65.5\%$ & $65.9\%$ $(+0.4)$ & $65.8\%$ $(+0.3)$ & $62.3\%$ $(-3.2)$ \\    
	 \bottomrule
\end{tabular}
%}
\label{tab:ablation-omp}
\caption{Accuracies for the ablation studies for one-shot magnitude pruning (OMP) at initialization.
Scores issued by OMP are represented by $s$. 
The standard version of OMP is marked with *.
Numbers in parentheses are the change in accuracy from the standard version.}
\end{table}


\subsection{SNIP}

Table \ref{tab:ablation-snip} below conducts the ablations for SNIP at initialization.
The analysis from OMP also applies to SNIP.
It is possible to randomly shuffle the pruning masks found at initialization and to randomly reinitialize the pruned network without substantial change in accuracy.
This means that, at initialization, SNIP is identifying only layerwise proportions in which to prune the network.
It is not identifying the specific sparse structure within each pruned layer or the specific initial weights to retain.
SNIP correctly determines that high-scoring parameters are more important to final accuracy than low-scoring parameters, but it is possible that pruning high-scoring weights simply selects poor layerwise proportions in which to prune the network.

\begin{table}[h]
%\resizebox{\textwidth}{!}{%
\centering
\small
\begin{tabular}{l | c c c c c}
    \toprule
    Name & Sparsity & Lowest $s$* & Lowest $s$ (Shuffled) & Lowest $s$ (Reinit) & Highest $s$ \\ \midrule
    \multirow{3}{*}{VGG-19}
	 & $90\%$ & $93.5\%$ & $93.3\%$ $(-0.2)$ & $93.4\%$ $(-0.1)$ & $51.6\%$ $(-41.9)$ \\
	 & $95\%$ & $93.4\%$ & $93.2\%$ $(-0.2)$ & $93.1\%$ $(-0.3)$ & $10.0\%$ $(-83.4)$ \\
	 & $98\%$ & $42.7\%$ & $55.8\%$ $(+13.1)$ & $40.4\%$ $(-2.3)$ & $10.0\%$ $(-32.7)$ \\
	 \midrule
    \multirow{3}{*}{WRN-32-2}
	 & $90\%$ & $92.5\%$ & $92.5\%$ $(+0.0)$ & $92.3\%$ $(-0.2)$ & $11.8\%$ $(-80.7)$ \\
	 & $95\%$ & $91.0\%$ & $91.1\%$ $(+0.1)$ & $90.7\%$ $(-0.3)$ & $10.0\%$ $(-81.0)$ \\
	 & $98\%$ & $87.7\%$ & $88.0\%$ $(+0.3)$ & $87.7\%$ $(+0.0)$ & $11.7\%$ $(-76.0)$ \\
	 \midrule
    \multirow{3}{*}{ResNet-50}
	 & $60\%$ & $74.2\%$ & $74.2\%$ $(+0.0)$ & $74.1\%$ $(-0.1)$ & $65.6\%$ $(-8.6)$ \\
	 & $80\%$ & $71.1\%$ & $71.2\%$ $(+0.1)$ & $71.2\%$ $(+0.1)$ & $19.7\%$ $(-51.4)$ \\
	 & $90\%$ & $64.7\%$ & $66.4\%$ $(+1.7)$ & $65.7\%$ $(+1.0)$ & $0.1\%$ $(-64.6)$ \\
	 \bottomrule
\end{tabular}
%}
\label{tab:ablation-snip}
\caption{Accuracies for the ablation studies for SNIP at initialization.
Scores issued by SNIP are represented by $s$. 
The standard version of SNIP is marked with *.
Numbers in parentheses are the change in accuracy from the standard version.}
\end{table}

\subsection{GraSP}

Table \ref{tab:ablation-grasp} below conducts the ablations for GraSP at initialization.
Like OMP and SNIP, it is possible to randomly shuffle the GraSP pruning masks found at initialization and to randomly reinitialize the pruned network without substantial change in accuracy.
This means that, at initialization, GraSP is identifying only layerwise proportions in which to prune the network.

Unlike OMP and SNIP, GraSP produces a signed score, where a positive score means removing a parameter improves gradient flow and a negative score means removing a parameter reduces gradient flow.
By the interpretation of \citet{wang2020picking}, it is beneficial to prune those parameters that most improve (or least reduce) gradient flow; that is, those parameters with the lowest scores are the most important.
However, the data in Table \ref{tab:ablation-grasp} does not support this interpretation: pruning parameters with the lowest scores does not affect accuracy.
In other words, it is just as effective to prune with the intention of destroying gradient flow (according to the GraSP scores) as it is to prune with the intention of ``preserving gradient flow.''

In light of these results, we attempted one further ablation: pruning scores with the lowest magnitudes.
Since it is equally effective to prune the lowest or highest scores, we hypothesized that the magnitude of the scores may also be a useful signal.
Indeed, we find that performance slightly improves when using the lowest magnitude scores in this way.
However, pruning the highest magnitude scores results in significant drops in accuracy.

We conclude that, although the GraSP scores do extract useful information from the network, the justification for the scores provided by \citet{wang2020picking} does not match the results in Table \ref{tab:ablation-grasp}.

\begin{table}[h]
\resizebox{\textwidth}{!}{%
\begin{tabular}{l | c c c c c c c}
    \toprule
    Name & Sparsity & Highest $s$* & Highest $s$ (Shuffled) & Highest $s$ (Reinit) & Lowest $s$ & Lowest $|s|$ & Highest $|s|$ \\ \midrule
    \multirow{3}{*}{VGG-19}
	 & $90\%$ & $92.8\%$ & $92.9\%$ $(+0.1)$ & $92.9\%$ $(+0.1)$ & $92.8\%$ $(+0.0)$ & $93.2\%$ $(+0.4)$ & $67.5\%$ $(-25.3)$ \\
	 & $95\%$ & $92.5\%$ & $92.5\%$ $(+0.0)$ & $92.6\%$ $(+0.1)$ & $92.4\%$ $(-0.1)$ & $92.9\%$ $(+0.4)$ & $37.0\%$ $(-55.5)$ \\
	 & $98\%$ & $91.9\%$ & $91.8\%$ $(-0.1)$ & $91.8\%$ $(-0.1)$ & $91.7\%$ $(-0.2)$ & $92.1\%$ $(+0.2)$ & $10.0\%$ $(-81.9)$ \\
	 \midrule
    \multirow{3}{*}{WRN-32-2}
	 & $90\%$ & $92.2\%$ & $92.2\%$ $(+0.0)$ & $92.2\%$ $(+0.0)$ & $92.2\%$ $(+0.0)$ & $92.4\%$ $(+0.2)$ & $31.3\%$ $(-60.9)$ \\
	 & $95\%$ & $90.9\%$ & $91.1\%$ $(+0.2)$ & $91.3\%$ $(+0.4)$ & $91.1\%$ $(+0.2)$ & $91.2\%$ $(+0.3)$ & $18.7\%$ $(-72.2)$ \\
	 & $98\%$ & $88.3\%$ & $88.5\%$ $(+0.2)$ & $88.4\%$ $(+0.1)$ & $88.4\%$ $(+0.1)$ & $88.3\%$ $(+0.0)$ & $11.6\%$ $(-76.7)$ \\
	 \midrule
    \multirow{3}{*}{ResNet-50}
	 & $60\%$ & $73.4\%$ & $73.6\%$ $(+0.2)$ & $73.6\%$ $(+0.2)$ & $73.3\%$ $(-0.1)$ & $74.1\%$ $(+0.7)$ & $69.7\%$ $(-3.7)$ \\
	 & $80\%$ & $71.0\%$ & $70.8\%$ $(-0.2)$ & $71.1\%$ $(+0.1)$ & $70.7\%$ $(-0.3)$ & $71.6\%$ $(+0.6)$ & $63.8\%$ $(-7.2)$ \\
	 & $90\%$ & $67.3\%$ & $67.3\%$ $(+0.0)$ & $67.2\%$ $(-0.1)$ & $66.8\%$ $(-0.5)$ & $67.8\%$ $(+0.5)$ & $52.2\%$ $(-15.1)$ \\
	 \bottomrule
\end{tabular}
}
\label{tab:ablation-grasp}
\caption{Accuracies for the ablation studies for GraSP at initialization.
Scores issued by GraSP are represented by $s$. 
The standard version of GraSP is marked with *.
Numbers in parentheses are the change in accuracy from the standard version.
This table includes an additional ablation where we prune parameters with the lowest-magnitude scores.}
\end{table}


==> appendices/concurrent-work-policy.tex <==
\section{ICLR 2021 Concurrent Work Policy}
\label{app:concurrent-work-policy}

According to correspondence with the ICLR 2021 program chairs:

\emph{We will follow the NeurIPS policy of treating papers concurrent if they are published in the two months prior to our paper deadline. So you will not be responsible for comparing with papers published on or after Aug 2.}

==> appendices/concurrent.tex <==
\section{Comparison to Concurrent Work}
\label{app:concurrent}

Concurrently and independently, \citet{su2020sanity} conducted shuffling ablations on SNIP and GraSP.
According to emails with the ICLR program chairs, ICLR ``follow[s] the NeurIPS policy of treating papers concurrent if they are published in the two months prior to our paper deadline.'' This means that we are ``not...responsible for comparing with papers published on or after Aug 2.'' The paper we discuss here was released on arXiv on Sep 22 and will not be published until NeurIPS occurs Dec 7, so it qualifies as concurrent work.
However, we include this comparison for the sake of rigor.\vspace{-1mm}


\textbf{Similarities in findings.} Our findings overlap with those of \citeauthor{su2020sanity} in the following ways:

\begin{itemize}[leftmargin=1em,itemsep=1pt,parsep=1pt,topsep=0pt,partopsep=0pt]
    \item We perform ablations to understand the information that pruning methods extract at initialization.
    \item We find that SNIP and GraSP maintain the same accuracy under the shuffling ablation.
    \item We show a ``zero-shot'' way to reach accuracy similar to SNIP and GraSP by selecting appropriate layer-wise pruning rates and pruning randomly.\footnote{While the ``zero-shot'' approach of \citeauthor{su2020sanity}~involves picking arbitrary per-layer pruning proportions based on depth, we find that we can simply use the proportions implicitly provided by the Kaiming variance-scaled initialization without additional work. We find this because we include magnitude pruning at initialization.}
\end{itemize}

\textbf{Differences in findings.} Our findings are distinct from those of \citeauthor{su2020sanity}~in the following ways:

\begin{itemize}[leftmargin=1em,itemsep=1pt,parsep=1pt,topsep=0pt,partopsep=0pt]
    \item In addition to SNIP and GraSP, we also show that these results hold for magnitude pruning, SynFlow, and iterative SNIP (Appendix \ref{app:iterative-snip}).
    \item We compare these methods at 14-18 sparsities (vs. 3 in \citeauthor{su2020sanity}) and include baselines (random pruning and magnitude after training).
          This allows us to reach the broader conclusions about the state of the art in pruning at initialization in Section \ref{sec:baselines}.
    \item We perform reinitialization\footnote{In their methodology, \citeauthor{su2020sanity}~mention an experiment where weights (but not masks) are shuffled within each layer in a manner similar to reinitialization. However, they do not perform this ablation on SNIP or GraSP.} and inversion ablations, and we show the practical value of ablations by using them to diagnose and improve GraSP (inversion) and SynFlow (neuron collapse).
    \item We show that the performance of the pruning methods improves only gradually if pruning occurs later in training, and we perform ablations on the pruning methods after training (Appendix \ref{app:ablations-after}).
\end{itemize}

\textbf{Differences in conclusions.}
These different findings lead us to different conclusions.
\citeauthor{su2020sanity}~conclude that the shuffling results ``cast[s] doubt on whether the[] individual connections in the pruned subnetwork [are] crucial'' and that ``the architecture of the pruned network may only have limited impact on the final performance.''\footnote{Although it is unclear in the paper, we presume \citeauthor{su2020sanity}~intend these claims to be specific to SNIP and GraSP rather than to apply to pruning in general (where there are known counterexamples, e.g., Appendix \ref{app:ablations-after}).}
We conclude more broadly that the ablations imply limitations inherent to these methods or to pruning at initialization.
We are able to draw this conclusion using the baseline of magnitude pruning after training, which (a) reaches higher accuracy and (b) is not robust to ablations.
This shows that there are indeed settings for which the pruned architecture matters and that there may be a connection between sensitivity to the ablations and accuracy.

\textbf{Differences in breadth.} Our findings are broader in the following ways:
\begin{itemize}[leftmargin=1em,itemsep=1pt,parsep=1pt,topsep=0pt,partopsep=0pt]
    \item We study more early pruning methods (SynFlow, magnitude, iterative SNIP).
    \item We include baselines (random, magnitude after training), neither of which are in \citeauthor{su2020sanity}\footnote{\citeauthor{su2020sanity}~include two experiments that they describe as lottery tickets. The first (which they call LT) involves rewinding to initialization, which is known to perform poorly on the networks that they study \citep{frankle2020lottery}. The second (which they call Learning Rate Rewinding after \citet{Renda2020Comparing}) is similar to our LTR baseline, although they do not specify the specific rewinding iterations that they use.}
    \item We include experiments on ResNet-50 on ImageNet, larger-scale than the CIFAR-10 and TinyImageNet experiments in \citeauthor{su2020sanity}
    \item We conduct our main experiments at between 14 and 18 different sparsities. \citeauthor{su2020sanity}~conduct ablations at five sparsities and compare between methods at three sparsities.
\end{itemize}

% \textbf{Differences in findings.} We make the following findings that do not appear in \citeauthor{su2020sanity}:
% \vspace{-2mm}
% \begin{itemize}[leftmargin=1em,itemsep=1pt,parsep=0pt,topsep=0pt,partopsep=0pt]
%     \item We explicitly compare all early pruning methods to each other and to the two baselines (Section \ref{sec:baselines}).
%     Because we use so many sparsities, we are able to reach broader conclusions about the pruning methods.
%     For example, we find that no single method is SOTA, SNIP generally performs well, GraSP performs relatively better at extreme sparsities, and magnitude pruning is surprisingly competitive.
%     We are also able to make comparisons between matching and extreme sparsities; in the main body of their paper, \citeauthor{su2020sanity} include just one matching sparsity for one network.
%     \item In addition to SNIP and GraSP, we find that SynFlow and magnitude are robust to shuffling.
%     \item While the ``zero-shot'' approach of \citeauthor{su2020sanity}~involves picking arbitrary per-layer pruning proportions based on depth, we find that we can simply use the proportions implicitly provided by the Kaiming variance-scaled initialization scheme without additional work.
%     \item We find that SNIP, GraSP, and SynFlow are robust to initialization changes that hurt magnitude.
%     \item We find that SynFlow improves when shuffling and attribute this to neuron collapse.
%     \item We include the reinitialization\footnote{In their methodology, \citeauthor{su2020sanity}~mention an experiment where weights (but not masks) are shuffled within each layer in a manner similar to reinitialization. However, they do not perform this ablation on SNIP or GraSP.} and inversion ablations. We find that all early pruning methods we consider are robust to reinitialization and that GraSP is robust to inversion.
%     \item We suggest an improved version of GraSP based on the results of the inversion experiment.
%     \item We investigate the performance of the early pruning methods throughout training (Section \ref{sec:after}) and perform ablations on all methods \emph{after} training (Appendix \ref{app:ablations-after}). We find that these methods improve only gradually early in training, underperforming LTR.
% \end{itemize}


==> appendices/tables.tex <==
\section{Tables of Numbers}

To facilitate easier comparisons and replication in the future, we have included tables of all of the numbers that went into our plots.
All numbers are mean $\pm$ stddev over five replicates (CIFAR-10) or three replicates (TinyImageNet and ImageNet).
